Parallax: Sparsity-aware Data Parallel Training of Deep Neural Networks

The employment of high-performance servers and GPU accelerators for training deep neural network models have greatly accelerated recent advances in deep learning (DL). DL frameworks, such as TensorFlow, MXNet, and Caffe2, have emerged to assist DL researchers to train their models in a distributed manner. Although current DL frameworks scale well for image classification models, there remain opportunities for scalable distributed training on natural language processing (NLP) models. We found that current frameworks show relatively low scalability on training NLP models due to the lack of consideration to the difference in sparsity of model parameters. In this paper, we propose Parallax, a framework that optimizes data parallel training by utilizing the sparsity of model parameters. Parallax introduces a hybrid approach that combines Parameter Server and AllReduce architectures to optimize the amount of data transfer according to the sparsity. Experiments show that Parallax built atop TensorFlow achieves scalable training throughput on both dense and sparse models while requiring little effort from its users. Parallax achieves up to 2.8x, 6.02x speedup for NLP models than TensorFlow and Horovod with 48 GPUs, respectively. The training speed for the image classification models is equal to Horovod and 1.53x faster than TensorFlow.

==> Makefile <==
TEXFILE=parallax.tex
TARGET=parallax
TEXFILES=$(wildcard *.tex)
BIBFILES=parallax.bib
FIGFILES=$(wildcard figures/*.pdf) $(wildcard figures/*.eps)

all: ${TARGET}.pdf

${TARGET}.pdf: ${TEXFILES} ${BIBFILES} ${FIGFILES} ${TARGET}.bbl
	( \
	pdflatex $(TARGET).tex; \
	while grep -q "Rerun to get cross-references right." $(TARGET).log; \
	do \
		pdflatex $(TARGET).tex; \
	done \
	)

${TARGET}.bbl: ${TARGET}.bib
	pdflatex ${TARGET}.tex
	bibtex ${TARGET}
	pdflatex ${TARGET}.tex
	pdflatex ${TARGET}.tex

.PHONY: clean
clean:
	rm -f \
	$(TEXFILE:.tex=.aux) \
	$(TEXFILE:.tex=.log) \
	$(TEXFILE:.tex=.out) \
	$(TEXFILE:.tex=.dvi) \
	$(TEXFILE:.tex=.pdf) \
	$(TEXFILE:.tex=.thm) \
	$(TEXFILE:.tex=.bbl) \
	$(TEXFILE:.tex=.blg) \
	$(TEXFILE:.tex=.ps) \
	$(TEXFILE:.tex=.ent) \
	latex.out/* \
	figures/*-eps-converted-to.pdf

.PHONY: build
build:
	@bin/latexrun $(TARGET)


==> scalability.tex <==
\section{Performance Tuning on \texttt{Weight}} \label{sec:scalability}
\tool tunes performance on each \texttt{Weight} that is a unit of computaion and communication in DL frameworks.
\texttt{Weight}s activiated independently according to what layers or operations are computed in a specific time.
As a result, performance tuning on each \texttt{Weight} improves overall scalabiltiy of distributed training.
\tool adapts two novel techniques for the performance tuning: hybrid communication and automatic partitioning for large \texttt{Weight}s.

{\subsection{Hybrid Communication} \label{subsec:hybrid}
As shown in Table~\ref{table:model_dataset}, PS and P2P communication mechanisms have their strengths.
PS communication performs better for sparse models, while P2P communication shows better performance for dense models. This observation motivates the hybridization of the two mechanisms to achieve the best of both worlds. We introduce hybrid communication, a new communication mechanism that utilizes P2P communication for dense parameters and PS communication for sparse parameters.

Table~\ref{table:data_transfer} shows the estimated amount of data transfer for a single GPU when a specific communication method is used.
For dense parameters, the amount is similar for both mechanisms: $2b$ bytes for PS and $2 (N - 1) b / N$ bytes for P2P, where $b$ is the parameter size in bytes, and $N$ is the number of GPUs.
In PS communication, each GPU sends and receives $2b$ bytes of data in a single iteration.
This formula is derived from the fact that each GPU reads $b$ bytes of parameters from servers for feedforward and backpropagation and produces $b$ bytes of gradients.
On the other hand, each GPU in P2P communication needs gradients generated from all GPUs to update parameter replicas; thus, each GPU sends $b$ bytes of data to $N - 1$ GPUs (total $(N - 1)b$ bytes) and receives $(N - 1)b$ bytes from other GPUs. 
However, employing an efficient ring-based \texttt{AllReduce} algorithm~\cite{ring} reduces the amount of data transfer to $2 (N - 1) b / N$. 
With the algorithm, each GPU sends and receives $b/N$ bytes for $2(N - 1)$ communication steps, gradients are aggregated for the first $(N-1)$ communication steps, and the aggregated values are broadcasted for the next $(N - 1)$ communication steps. 
Since both PS and P2P transfer the similar amount of data ($2b$ and $2 (N - 1)/N b$  bytes), communication speed highly depends on the optimization of their implementations. 

For example, NVIDIA's library for collective communication (NCCL~\cite{nccl}) provides highly optimized \texttt{AllReduce} with the ring algorithm.
NCCL is aware of the topology of hardware, such as PCI and network interfaces, to optimize communication between GPUs and between machines.
As a result, it achieves high performance and scales well on dense models such as ResNet-50~\cite{resnet}, Inception-v3~\cite{inception}, and VGG-16~\cite{vgg}, according to a recent study~\cite{horovod}. 
We also confirmed it with our experiments in Section~\ref{sec:evaluation}. Thus, \tool adopts P2P using NCCL for dense parameter communication.

Exchanging sparse parameters using P2P communication requires much more data transfer compared to PS communication. 
In PS communication, each GPU sends and receives $2\alpha b$ bytes of data in a single iteration, where $\alpha$ represents sparsity, which is the average ratio of activated parameters over all parameters.
Calculation of the amount of data transfer in PS is the same for both dense and parameters except $\alpha$, which is added because the only subset of sparse parameters ($\alpha b$) is necessary at each iteration.
For the P2P communication, \texttt{AllGatherv} is used for sparse parameters. Reducing the amount of data transfer as in \texttt{AllReduce} is not applicable to \texttt{AllGatherv} because \texttt{AllGatherv} aggregates gradients of each worker by appending them instead of adding values as in \texttt{AllReduce}. It results in the data transfer of $2 (N - 1) \alpha b$ bytes for a GPU.
Therefore, the amount of data transfer in P2P communication $(N-1)$ times larger than PS communication. 
As $N$ becomes large, the difference between the two communication methods becomes significant.

Thus, \tool introduces a hybrid communication mechanism (Figure~\ref{fig:hybrid}) as an optimization by applying P2P communication for dense parameters and PS communication for sparse parameters, so that each worker in a GPU has a replica of dense parameters, while a server process in each machine manages only sparse parameters and communicates with workers. If there are only dense parameters in a model, such as ResNet-50~\cite{resnet} and Inception-v3~\cite{inception}, the hybrid communication works same as P2P.

{\subsection{Paritioning of large \texttt{Weight}s} \label{subsec:partitioning}
Table~\ref{table:partitions} indicates the number of partitions($P$) for large \texttt{Weight}s hugely impacts on overall throughput.
The $P$ is gettting larger, the ability for parallel processing of \texttt{Weight} is increased results in speed-up. 
On the other hand, the overhead to manage partitioned \texttt{Weight}s offsets the ability. 
Figure~\ref{} shows the partition effects well for LM and NMT models. 
When the number of partitions is relatively small(less than X in LM and less than y in NMT), execution time is proportionally decreased according to the increase of $P$. 
However, the tendency is inversed on large partitions.

Finding the $P$ compromises both sides happy is a time-consuming process.
Thus, \tool finds the optimal value using sampling and learned model from sampled results to minimize the search overhead.
The sampling starts with $P$ as the number of machinses and collects execution time by doubling $P$ until it is increased or decreased less than 10\%. By searching only the performance is increased more than 10\%, \tool prevents the large sampling overhead compared to small gain from the optimal value. Then, the other side is searched by halving $P$ until the same condition.
This sampling results are ready for training a model because it holds for both positive and negative(or less effective than 10\%) effects according to $P$.

\tool builds a linear model to find optimal $P$ with three terms. 
The terms are a) a fixed cost term which represents the unavoidable computation time, b) the parallel execution and communication time accoding to $P$ and c) the overehad that scale as \texttt{Weight}s are more partitioned. 
The overall model to learn values for $\theta0$, $\theta1$ and $\theta2$ in the formula
\begin{equation}
exec\_time = 
\theta0 + \theta1 * \frac{1}{P} + \theta2 * P
\end{equation}
We trained the model using mean-squared error of the sampled time and prediction. 

The method has sampling overhead X\%, Y\% compared to the training time in LM and NMT respectively while the throughput is improved at most X\%, Y\% than the worst case and X\%, Y\% than the the best results during sampling.
It helps finding optimal $P$ for relatively large \texttt{Weight}s, which are embedding and its softmax paramters in LM and NMT, compared to the others.
If a model needs to find multiple $P$ values in a different scale, the method still can be applied for one by one(i.e., finding $P1$  and then searching for $P2$) even though the search overhead can be increased.
